Online Clustering of Bandits

We introduce a novel algorithmic approach to content recommendation based on adaptive clustering of exploration-exploitation ("bandit") strategies. We provide a sharp regret analysis of this algorithm in a standard stochastic noise setting, demonstrate its scalability properties, and prove its effectiveness on a number of artificial and real-world datasets. Our experiments show a significant increase in prediction performance over state-of-the-art methods for bandit problems.

==> abstract_intro.tex <==


\begin{abstract} 
%updated the abs to best fit the space and better considered description by shuai
We introduce a novel algorithmic approach to content-based recommendation system
% in interacting user scenarios (e.g., a social network) 
with the adaptive clustering of exploration-exploitation (``bandit") tradeoff strategies. 
We provide a sharp regret analysis of this algorithm in a standard stochastic 
noise setting, demonstrate its scalability properties, and 
prove its effectiveness on both a number of artificial and real-world datasets.
Our experiments show a significant increase in prediction performance
over state-of-the-art methods for bandit problems. 
%
\iffalse
********************
{\bf GZ: tentative}
Contextual bandit problems formalize the exploration-exploitation dilemma arising in several industrial applications, such as online advertisement and, more generally, recommendation systems.
In some of these applications such webpages personalization, the algorithm should learn a model for each user of the website starting with little or no information.
In practice, it is often the case that a user is not completely different from each other, and in general, it is often possible to find a small set of models those represents the preferences of all the users creating in this way a cluster of users for each model.

Unfortunately, the learner does not have any previous knowledge on the similarity among the users, on the candidate models or on the number of models those are necessary to represent all the users.
The only viable way for the learner to exploit this similarity is to learn a clusterization of the users while it learns the models, \textit{betting} on the fact that the number of distinct models will be much smaller than the total number of users.

In this paper we present an algorithm for learning similarity and sharing feedback among multiple linear bandit problems, while obtaining a regret bound that depends on the real number of clusters instead of on the number of users. 
The last part of the paper is dedicated to compare our algorithm with the state of the art algorithms for linear bandits.
*********************
\fi
\end{abstract} 

\vspace{-0.25in}



\section{Introduction}
%
\vspace{-0.05in}
Presenting personalized content to users is nowdays a crucial functionality for many online 
recommendation services. Due to the ever-changing set of available options, these services 
have to exhibit strong adaptation capabilities when trying to match 
%as much as possible the 
users' preferences. 
%In essence, 
Coarsely speaking, the underlying systems repeatedly learn a mapping between available content 
and users, the mapping being based on {\em context} information (that is, sets of features) which is 
typically extracted from both users and contents. 
The need to focus on content that raises the users' interest, 
combined with the need of exploring new content so as to globally improve users' experience, 
generates a well-known exploration-exploitation dilemma, which is commonly formalized as 
a multi-armed bandit problem~(e.g., \cite{lr85,ACF01,audibert:hal-00711069,CaronKLB12}). 
In particular, the contextual bandit methods~(e.g., \cite{Aue02,lz07,li2010contextual,chu2011contextual,
bogers2010movie,abbasi2011improved,cg11,ko11}, and references therein) 
have rapidly become a reference algorithmic technique for implementing adaptive recommender systems.

\vspace{-0.05in}
% new challenge: users are increasing in number, and interact
Within the above scenarios, the widespread adoption of online social networks, where users are 
engaged in technology-mediated social interactions (making product endorsement and word-of-mouth 
advertising a common practice), raises further challenges and opportunities to content recommendation 
systems: On one hand, because of the mutual influence among friends, acquaintances, business partners, 
etc., users having strong ties are more likely to exhibit similar interests, and therefore similar 
behavior. On the other hand, the nature and scale of such interactions calls for adaptive
algorithmic solutions which are also computationally affordable.

\vspace{-0.05in}
% two approaches: explicit networks and implicit networks
Incorporating social components into bandit algorithms can lead to a dramatic increase in the quality 
of recommendations. For instance, we may want to serve content to a group of users by taking advantage of 
an underlying network of social relationships among them. These social relationships can either be 
explicitly encoded in a graph, where adjacent nodes/users are deemed similar to one another, or implicitly
contained in the data, and given as the outcome of an inference process that recognizes similarities 
across users based on their past behavior. 
Examples of the first approach are the recent works~\cite{bes13,dkmc13,cgz13}, where
a social network structure over the users is assumed to be given that reflects actual interest similarities
among users -- see also \cite{cb13, valko2014spectral} for recent usage of social information to tackle the so-called 
``cold-start" problem. Examples of the second approach are the more traditional 
collaborative-filtering (e.g.,~\cite{skr99}), content-based filtering, and hybrid approaches (e.g.~\cite{b05}).
Both approaches have important drawbacks hindering their practical deployment. One obvious drawback
of the ``explicit network" approach is that the social network information may be misleading
%(e.g., ``is it really true that if we are friends in Facebook then we like the same books ?") 
(see, e.g., the experimental evidence reported by~\cite{dkmc13}), or simply unavailable. 
Moreover, even in the case when this information is indeed available and useful, 
the algorithmic strategies to implement the needed feedback sharing mechanisms might lead to severe 
scaling issues~\cite{cgz13}, especially when the number of targeted users is large.
A standard drawback of the ``implicit network" approach of traditional recommender systems 
is that in many practically relevant scenarios (e.g., web-based), content universe and popularity often 
undergo dramatic changes, making these approaches difficult to apply. 

\vspace{-0.05in}
In such settings, most notably in the relevant case 
when the involved users are many, it is often possible to identify 
a few subgroups or communities within which users share similar interests~\cite{rlkr06,bwdh12},
%~\cite{xlyxzyc05,rlkr06,bwdh12}, 
thereby greatly facilitating 
the targeting of users by means of {\em group} recommendations. Hence the system need not learn 
a different model for each user of the service, but just a single model for each group. 

\vspace{-0.05in}
In this paper, we initiate\footnote
{
The only paper we are aware of which has similar goals as ours is~\cite{bkm12}, though that 
paper apparently works under more restrictive assumptions.
} 
a theoretical and experimental investigation of adaptive clustering algorithms
for linear (contextual) bandits under the assumption that we have to serve content to a set of $n$ users 
organized into $m << n$ groups (or {\em clusters}) such that users within each group tend to provide
similar feedback to content recommendations. We give a $O(\sqrt{T})$ regret analysis holding in a standard
stochastically linear setting for payoffs where, importantly, the hidden constants in the big-oh 
depend on $m$, rather than $n$, as well as on the geometry of the user models within the different 
clusters.
%
The main idea of our algorithm is to use confidence balls of the users' models to both estimate user similarity, 
and to share feedback across (deemed similar) users. The algorithm adaptively interpolates between
the case when we have a single instance of a contextual bandit algorithm making the same predictions for all 
users and the case when we have $n$-many instances providing fully personalized recommendations.
We show that our algorithm can be implemented efficiently (the large $n$ scenario being of special concern here) 
by means of off-the-shelf data-structures relying on random graphs. Finally, we test our algorithm 
on medium-size synthetic and real-world datasets, often reporting a significant increase in prediction performance
over known state-of-the-art methods for bandit problems. 




\iffalse
In practice, it is often the case that the system does not need to learn a different model for each single user of the service, but it can just learn a model for each cluster of users with similar taste. 
This problem has somehow already been addressed in previous papers, assuming that side information from a social network among the users was provided to the algorithm (i.e., see \cite{}). 
Unfortunately, it is not always the case: in some cases there is not information available about the users except their current behavior, and even when the side information is available it may not provide good similarity information. %This will also address the problem of learning personalized models when the users interact with the service very few times.
Learning the similarity among the users while learning their preferences model is far from trivial.\\
In this work, we provide an algorithm for contextual bandits able to learn and leverage the similarity among the users. 

The main idea is to use the confidence balls of the users' models to estimate the similarity among the users and in this way allow the algorithm to share feedback among similar users.
This mechanism is implemented running a single contextual bandit algorithm for each cluster of users, using all the feedback obtained for all the predictions made for the users in the cluster.
Roughly speaking, the algorithm interpolates between the case where there is only one instance of a contextual bandits making predictions for all the users and the case where there is a single instance of a contextual bandit algorithm for each user.\\
In the last part of the paper, we present a comparison between the new algorithm and the state of the art linear bandit algorithms in a completely controlled environment.
Oftentimes our algorithm outperforms its competitors and it is never worse than the best among them.
\fi





==> experiments_icml.tex <==



\section{Experiments}\label{s:exp}
%
In this section, we compare our CLUB algorithm to known bandits algorithm baselines.
These baselines are versions of linear (i.e., ``contextual") upper-confidence bandit algorithms 
(e.g., the LinUCB family of algorithms~\cite{Aue02,chu2011contextual,li2010contextual,abbasi2011improved}, 
as well as some of their featureless (i.e., ``noncontextual") counterparts (e.g., UCB~\cite{ACF01} and 
UCB-V~\cite{audibert:hal-00711069}).


\subsection{Datasets}
%
We tested our algorithm and its competitors on both artificial and freely available 
real-world datasets.

\textbf{Artificial datasets.}
In order to validate our theoretical findings (Theorem \ref{t:regret}), we first generated synthetic datasets, so as to have
a more controlled experimental setting. We tested the relative performance of the algorithms 
along different axes: number of underlying clusters, balancedness of cluster size, and amount of payoff noise. 
We set the number $c_t$ of context vectors as $c_t = 10$ for all $t = 1, \ldots, T$, with horizon $T = 50,000$, 
the input dimension $d$ as $d = 50$, the total number $n$ of users as $n = 2,000$. 
For each cluster $V_j$ of users, we created a random 
unit norm vector $\bu_j \in \R^d$. All $d$-dimensional context vectors $\bx_{t,k}$
%
% For practical reasons we fixed the number of vectors per time step as 10, the number of dimensions of the 
% context vectors as 50 and the number of users as 2000.
% These values were picked with the aim to have a fair comparison under the constraint of limited 
% computational resources: the number of context vectors and dimensions are reasonable values for practical applications. 
%If they are too small the problem becomes kind of too easy, while if they are too big the requirements 
% in term of computational resources becomes unaffordable.
% The number of users and cluster was fixed in order to explore different practical situations.
%
have then been generated uniformly at random on the surface of the Euclidean ball.
The payoff value associated with cluster vector $\bu_j$ and context vector $\bx_{t,k}$ has been generated 
by perturbing the inner product $\bu_j^\top\bx_{t,k}$ through an additive white noise term $\epsilon$ drawn 
uniformly at random across the range $[-\sigma,\sigma]$. It is the value of $\sigma$ that determines the amount
of payoff noise. 
%
The two remaining parameters we wanted to control are the number of clusters $m$ and the clusters' relative size. 
We assigned to cluster $V_j$ a number of users $|V_j|$ calculated as\footnote
{
Since we cannot assign fractionary parts of users, we take the integer part in this formula, and then reassign 
the remaining users to the first cluster.
} 
$|V_j| = n\,\frac{j^{-z}}{\sum_{\ell=1}^m \ell^{-z}}$, $j = 1, \ldots, m$,
where the exponent $z$ ranges in \{0,1,2,3\}, so that $z = 0$ corresponds to equally-sized clusters, and 
$z = 3$ yields highly unbalanced cluster sizes.
Finally, the sequence of served users $i_t$ is generated uniformly at random over the $n$ users.



\begin{figure}
\begin{picture}(40,12)(40,12)
\begin{tabular}{l@{\hspace{-4.8pc}}l}
\includegraphics[width=0.37\textwidth]{plots/z0_numClus2_pNoise0-1.pdf}
& \includegraphics[width=0.37\textwidth]{plots/z0_numClus2_pNoise0-3.pdf}\\[-2.2in]
\includegraphics[width=0.37\textwidth]{plots/z0_numClus10_pNoise0-1.pdf}
& \includegraphics[width=0.37\textwidth]{plots/z0_numClus10_pNoise0-3.pdf}\\[-2.2in]
\end{tabular}
\end{picture}
\vspace{2.4in}
\caption{\label{fig:artificial0}Results on synthetic datasets. Each plot displays the behavior of 
the ratio of the current cumulative regret of the algorithm (``Alg") to the current cumulative regret
of RAN. In all plots, the blue curve is obtained when ``Alg" = ``CLUB", 
the red one when ``Alg" = ``LinUCB-IND", and the black one when ``Alg" = ``LinUCB-ONE". The cluster sizes 
are balanced ($z=0$). From left to right, payoff noise steps from $0.1$ to $0.3$, and from top to bottom 
the number of clusters jumps from $2$ to $10$.}
\vspace{-0.1in}
\end{figure}
%
\begin{figure}
\begin{picture}(40,52)(40,52)
\begin{tabular}{l@{\hspace{-4.8pc}}l}
\includegraphics[width=0.37\textwidth]{plots/z2_numClus2_pNoise0-1.pdf}
& \includegraphics[width=0.37\textwidth]{plots/z2_numClus2_pNoise0-3.pdf}\\[-2.2in]
\includegraphics[width=0.37\textwidth]{plots/z2_numClus10_pNoise0-1.pdf}
& \includegraphics[width=0.37\textwidth]{plots/z2_numClus10_pNoise0-3.pdf}
\end{tabular}
\end{picture}
\vspace{1.85in}
\caption{\label{fig:artificial2}Results on synthetic datasets in the case of unbalanced ($z=2$) cluster sizes. 
The rest is the same as in Figure \ref{fig:artificial0}.}
\vspace{-0.1in}
\end{figure}




\textbf{LastFM \& Delicious datasets.} 
These datasets are extracted from the music streaming service Last.fm and the
social bookmarking web service Delicious. 
The LastFM dataset contains $n = 1,\!892$ nodes, and $17,\!632$ items (artists), described by $11,\!946$ tags. 
This dataset contains information about the listened artists, and we used this information to 
create payoffs: If a user listened to an artist at least once the payoff is $1$, otherwise the payoff is $0$.
Delicious is a dataset with $n = 1,\!861$ users. There are $69,\!226$ items (URLs) described by $53,\!388$ tags. 
The payoffs were created using the information about the bookmarked URLs for each user: 
The payoff is $1$ if the user bookmarked the URL, otherwise the payoff is $0$.\footnote
{
Datasets and their full descriptions are available at \texttt{www.grouplens.org/node/462}.
} 
%Both datasets were created by the Information Retrieval group at Universidad Autonoma de Madrid for the 
%HetRec 2011 Workshop~\cite{hetrec} with the goal of investigating the usage of heterogeneous information in recommendation systems.
These two datasets are inherently different: on Delicious, payoffs depend on users more strongly 
than on LastFM, that is, there are more popular artists whom everybody listens to 
than popular websites which everybody bookmarks. The former is a ``few hits" scenario, the latter is 
a ``many niches" scenario. 
This makes a big difference in practice, and the choice of these two datasets 
allow us to make a more realistic comparison of recommendation techniques.
Preprocessing was carried out by closely following previous experimental settings, such as the one
described by \cite{cgz13}. In particular, we only retained the first 25 principal components of the context 
vectors resulting from a tf-idf representation of the available items, so that on both datasets $d=25$.
We generated random context sets $C_{i_t}$ of size $c_t = 25$ for all $t$ as follows. User index $i_t$
was again selected uniformly at random over the $n$ users, then we 
picked $24$ vectors at random from the available items, and one among those vectors with nonzero payoff for user 
$i_t$. Notice that this is needed if we want to avoid a meaningless comparison: With high probability, a purely 
random selection would result in payoffs equal to zero for all the context vectors in $C_{i_t}$.
We repeated this process $T = 50,\!000$ times for the two datasets.


\textbf{Yahoo dataset.} We extracted two datasets from the one 
adopted by the ``ICML 2012 Exploration and Exploitation 3 Challenge''
%\footnote
%{
%\texttt{explochallenge.inria.fr/category/challenge}
%} 
for news article recommendation, which is in turn provided by the ``Yahoo Webscope program''.
%\footnote{
%\texttt{webscope.sandbox.yahoo.com}
%} 
%about news recommendation. 
Each user is represented by a 136-dimensional binary feature vector, and
we took this feature vector as a proxy for the identity of the user (no other usage was made of these
feature vectors). We operated on the first week of data only. After removing ``zombie" users,
this gave rise to a dataset of $8,362,905$ records, corresponding to $n = 713,862$ distinct users.
The overall number of distinct news items turned out to be $323$, with a number $c_t$ of context vectors
that changes from round to round, with a maximum of $51$, and a median of $41$. 
The news items have no features, so that they
have been represented as $d$-dimensional {\em versors}, with $d = 323$. 
Payoff values $a_t$ are either 1 or 0 depending on whether
the logged web system which these data refer to has observed a positive (click) or negative (no-click) 
feedback from the user in the current round. 
We then extracted the two datasets ``5k users"
and ``18k users" by filtering out users that have occurred less than $100$ times and less than $50$ times, 
respectively, resulting in $1,947,041$ and $2,829,308$ records, respectively.
However, because the system's recommendation need not coincide
with the recommendation issued by the algorithms we tested, we could only retain the records on which
the two recommendations were indeed the same.
Because records are discarded on the fly, the actual number of retained records changes 
across algorithms, but it is about $50,000$ for the ``5k users" version and  about $70,000$ for the 
``18k users" version. 




\subsection{Algorithms}
%
We contrasted CLUB with two main competitors: LinUCB-ONE and LinUCB-IND. 
Both competitors are versions of the LinUCB-like algorithm described by \cite{cgz13}
(see also \cite{Aue02,chu2011contextual,li2010contextual,abbasi2011improved} and references therein).
Specifically, whereas LinUCB-ONE allocates a single instance of LinUCB across all users (thereby making the same
prediction for all users), LinUCB-IND (``LinUCB INDependent") allocates an independent instance of LinUCB
to each user, thereby making predictions in a fully personalised fashion.
On the Yahoo dataset, we tested the featureless version of the LinUCB-like algorithm in~\cite{cgz13}, which 
is essentially a version of the UCB1 algorithm in \cite{ACF01}. 
The corresponding ONE and IND versions are denoted by UCB-ONE and UCB-IND, respectively. 
On this dataset, we also tried a single instance of UCB-V across all users, 
the winner of the ICML 2012 Exploration and Exploitation 3 Challenge.
Finally, all algorithms have also been compared (one way or another -- see below) to the trivial 
baseline that picks the item within $C_{i_t}$ fully at random. This baseline is denoted by RAN.

As for parameter tuning, CLUB was run with $p = \frac{3\,\log n}{n}$, so as to be reasonably confident
that the initial graph is connected.
In fact, after each random generation of the graph, we checked for its 
connectedness, and repeated its generation until the graph happened to be connected.\footnote
{
Our results are averaged over 5 random initial graphs, but this randomness  
turned out to be of minor influence to CLUB's performance.
}
All algorithms (but RAN) require parameter tuning: an exploration-exploitation tradeoff parameter
which is common to all algorithms (in Figure \ref{alg:club}, this is the $\alpha$ parameter), 
and the edge deletion parameter $\alpha_2$ in CLUB.
On the synthetic datasets, as well as on the LastFM and Delicious datasets, we tuned these parameters
by picking the best setting (as measured by cumulative regret) after the first $t_0 = 5,000$ rounds, and 
then sticked to those values for the remaining $T-t_0 = 45,000$ rounds. On the Yahoo dataset, 
this optimal tuning was done within the first $t_0 = 100,000$ records, corresponding
to a number of retained records between $4,350$ and $4,450$ acrosss different algorithms.\footnote
{
{\bf CG:} In our cumulative behavior plots, we do still take this initial stage into account ...
}



\subsection{Results}
%
Our results are summarized in
% \footnote
% {
% For space limitations, we can only provide a few such figures here.
% } 
Figures \ref{fig:artificial0}, \ref{fig:artificial2}, \ref{fig:last_del}, and \ref{fig:yahoo}.
On the synthetic datasets (Figures \ref{fig:artificial0} and \ref{fig:artificial2}) and  
the LastFM and Delicious datasets (Figure \ref{fig:last_del}) we measured the ratio of 
the cumulative regret of the algorithm (either CLUB or LinUCB-IND or LinUCB-ONE)
to the cumulative regret of the random predictor RAN (so that the lower the better).
On the synthetic datasets, we did so under combinations of number of clusters, payoff noise, 
and cluster size balancedness.
On the Yahoo dataset, because the only available payoff value is the one associated with the 
item recommended in the logs, we instead measured the Clickthrough Rate (CTR), namely the fraction
of times we observe $a_t = 1$ out of the number of retained records so far (so that the higher 
the better). This experimental setting is in line with previous ones (e.g., \cite{li2010contextual})
and, by the way data have been prepared, gives rise to a reliable estimation of actual CTR behavior
under the tested experimental conditions.
%
\begin{figure}
\begin{picture}(62,15)(62,15)
\begin{tabular}{l@{\hspace{-10.7pc}}l}
\includegraphics[width=0.51\textwidth]{lastfm.pdf}
& \includegraphics[width=0.51\textwidth]{delicious.pdf}
\end{tabular}
\end{picture}
\vspace{0.9in}
\caption{\label{fig:last_del}Results on the LastFM (left) and the Delicious (right) datasets.
The two plots display the behavior of the ratio of the current cumulative regret of the algorithm 
(``Alg") to the current cumulative regret of RAN, where ``Alg" is either ``CLUB" or ``LinUCB-IND" 
or ``LinUCB-ONE".}
%\vspace{-0.2in}
\end{figure}
%

Our experiments are still a bit preliminary. Yet, some trends can alrealy be spotted:
\textbf{On the synthetic datasets}, CLUB always outperforms its competitors, the gap
getting larger as we either decrease the number of underlying clusters or we make the clusters sizes more
and more unbalanced. Moreover, CLUB can clearly interpolate between the two competitors taking, in a sense, 
the best of both.
%
\textbf{On the ``few hits" } scenario provided by LastFM, CLUB is again outperforming
both of its competitors. However, this is not happening in the \textbf{``many niches"} case
delivered by the Delicious dataset, where CLUB is clearly outperformed by LinUCB-IND. 
%GZ: we shuld try CLUB with initial graph empty
The proposed alternative of CLUB that starts with an empty graph may be an effective alternative in this case.
%
On the \textbf{Yahoo datasets} we extracted, CLUB tends to outperform its competitors, when
measured by CTR curves, thereby showing that clustering users solely based on past behavior 
can be beneficial.

%
In general, CLUB seems to benefit from situations where it is not immediately 
clear which is the winner between the two extreme solutions (Lin)UCB-ONE and (Lin)UCB-IND,
and an adaptive interpolation between these two is needed.

% \item When the cluster are unbalanced (as often happen in the real world) CLUB 
% performs better than its competitors
% \item CLUB can split more aggressively when the payoff noise is low
% \item As we explained in the previous sections CLUB can interpolate between 
% the single predictor and $|V|$ independent predictors: in some extreme cases it 
% has the same behaviour of one of them.
% \item In general CLUB benefits from situations where it is not immediatly clear 
% which is the winner between LinUCB-SIN and LinUCB-IND









\begin{figure}
\begin{picture}(45,25)(45,25)
\begin{tabular}{l@{\hspace{-7.7pc}}l}
\includegraphics[width=0.43\textwidth]{yahoo100.pdf}
& \includegraphics[width=0.432\textwidth]{yahoo50.pdf}
\end{tabular}
\end{picture}
\vspace{0.9in}
\caption{\label{fig:yahoo}Results on the Yahoo datasets. 
Both plots report Clickthrough Rate (CTR) over time, i.e., the fraction of times 
the algorithm gets payoff one out of the number of retained records so far.}
\vspace{-0.2in}
\end{figure}






==> implementation.tex <==


\subsection{Implementation}\label{sa:implementation}
%
As we said in the main text, in implementing the algorithm in Figure \ref{alg:club}, 
the reader should keep in mind that it is reasonable to
expect $n$ (the number of users) to be quite large, $d$ (the number of features of each item) to be relatively small,
and $m$ (the number of true clusters) to be very small compared to $n$. 
Then the algorithm can be implemented by storing a least-squares estimator $\bw_{i,t-1}$ 
at each node $i \in V$, an aggregate least squares estimator $\bbw_{\hj_t,t-1}$ for each current cluster 
$\hj_t \in \{1,\ldots, m_t\}$, and an extra data-structure which is able to perform decremental dynamic connectivity.
Fast implementations of such data-structures are those studied by~\cite{Tho97,kkm13}
(see also the research thread referenced therein). In particular, in \cite{Tho97} (Theorem 1.1 therein)
it is shown that a randomized construction exists that maintains a spanning forerst which, given an initial
undirected graph $G_1 = (V,E_1)$, is able to perform edge deletions and answer connectivity queries of the form 
``Is node $i$ connected to node $j$" in expected total time 
$O\left(\min\{|V|^2, |E_1|\,\log |V|\} + \sqrt{|V|\,|E_1|}\,\log^{2.5} |V|\right)$ for $|E_1|$ deletions. 
Connectivity queries and deletions can be 
interleaved, the former being performed in {\em constant} time. Notice that when we start off from the full graph, 
we have $|E_1| = O(|V|^2)$, so that the expected amortized time per query becomes constant. On the other hand, 
if our initial graph has
% \footnote
% {
% It is well known that a random Erdos-Renyi graph where $p = \frac{\log |V|}{|V|}$ is the independent probability that
% two nodes are connected will be a connected graph with high probability, as $|V| \rightarrow \infty$. Hence, 
% if the initial graph $G_1 = (V,E_1)$ is an Erdos-Renyi graph with $|E_1| = \Omega(|V|\,\log |V|)$, then $G_1$ 
% is likely to be a connected graph.
% } 
$|E_1| = O(|V|\,\log |V|)$ edges, then the expected amortized time per query is $O(\log^2 |V|)$. This becomes 
$O(\log^{2.5} |V|)$ if the initial graph has $|E_1| = O(|V|)$.
In addition, we maintain an $n$-dimensional vector $\ci$ containing, for each node $i \in V$, 
the index $j$ of the current cluster $i$ belongs to.

With these data-structures handy, we can implement our algorithm as follows.
% and the set of connected components of the current graph $G_t$. 
% The least-squares estimators are maintained
% by an inverse matrix $M^{-1}_{i,t}$ (or $\bM^{-1}_{j,t}$) and a vector $\bb_{i,t}$ 
After receiving $i_t$, computing $j_t$ is $O(1)$ (just by accessing $\ci$). Then, computing $k_t$ can be done
in time $O(d^2)$ (matrix-vector multiplication, executed $c_t$ times, assuming $c_t$ is a constant). 
Then the algorithm directly updates $\bb_{i_t,t-1}$ and  $\bbb_{\hj_t,t-1}$, as well
as the inverses of matrices $M_{i_t,t-1}$ and 
$\bM_{\hj_t,t-1}$, which is again $O(d^2)$, using standard formulas for rank-one adjustment of inverse matrices.
In order to prepare the ground for the subsequent edge deletion phase,
it is convenient that the algorithm also stores at each node $i$ matrix $M_{i,t-1}$ (whose time-$t$ update is again $O(d^2)$). 

Let $\delete(i,\ell)$ and $\connected(i,\ell)$ be the two operations delivered by the decremental dynamic connectivity
data-structure.
Edge deletion at time $t$ corresponds to cycling through all nodes $\ell$ such that $(i_t,\ell)$ is an existing edge.
The number of such edges is on average equal to the average degree of node $i_t$, which is $O\left(\frac{|E_1|}{n}\right)$,
where $|E_1|$ is the number of edges in the initial graph $G_1$.
Now, if $(i_t,\ell)$ has to be deleted (each the deletion test being $O(d)$), 
then we invoke $\delete(i_t,\ell)$, and then $\connected(i_t,\ell)$. If $\connected(i_t,\ell)$ = ``no", 
this means that the current cluster $\hat V_{j_t,t-1}$ has to split into two new clusters as a consequence of the 
deletion of edge $(i_t,\ell)$.
The set of nodes contained in these two clusters correspond to the two sets
%
\begin{align*}
&\{ k \in V\,:\, \connected(i_t,k) = ``yes"\},\\ 
&\{ k \in V\,:\, \connected(\ell,k) = ``yes"\}`,
\end{align*}
%
whose expected amortized computation {\em per node} is $O(1)$ to $O(\log^{2.5}n)$
(depending on the density of the initial graph $G_1$). We modify the $\ci$ vector accordingly, 
but also the aggregate least squares estimators. This is because $\bbw_{\hj_t,t-1}$ 
(represented through $\bM^{-1}_{\hj_t,t}$ and $\bbb_{\hj_t,t}$) has to be spread over the two newborn clusters.
This operation can be
performed by adding up all matrices $M_{i,t}$ and all $\bb_{i,t}$, over all $i$ belonging to each of the
two new clusters
(it is at this point that we need to access $M_{i,t}$ for each $i$),
and then inverting the resulting aggregate matrices. This operation takes $O(n\,d^2 + d^3)$.
However, as argued in the comments preceeding the statement of 
Theorem \ref{t:regret} below, with high
probability the number of current clusters $m_t$ can never exceed $m$, so that with the 
same probability this operation is only
performed at most $m$ times throughout the learning process.
Hence in $T$ rounds we have an overall (expected) running time 
%
\begin{align}
O\Biggl(&T\,\left(d^2 + \frac{|E_1|}{n}\,d\right) + m\,(n\,d^2 + d^3) + |E_1|\notag\\ 
&+ \min\{n^2, |E_1|\,\log n\} + \sqrt{n\,|E_1|}\,\log^{2.5} n\Biggl)~.\label{e:runningtime}
\end{align}
%
%where $|E_1|$ is the number of edges in the initial graph $G_1$. 
Notice that the above is $n\cdot{\mbox{poly}}(\log n)$,
if so is $|E_1|$. In addition, if $T$ is large compared to $n$ and $d$, the average running time per round
becomes $O(d^2 + d\cdot{\mbox{poly}}(\log n))$.

As for memory requirements, we need to store two $d\times d$ matrices and one $d$-dimensional 
vector at each node, one $d\times d$ matrix and one $d$-dimensional vector for each current cluster, vector 
$\ci$, and the data-structures allowing for fast deletion and connectivity tests. Overall, these data-structures 
do not require more than $O(|E_1|)$ memory to be stored, so that this implementation
takes $O(n\,d^2 + m\,d^2 + |E_1|) = O(n\,d^2+|E_1|)$, where we again relied upon the $m_t \leq m$ condition.
Again, this is $n\cdot{\mbox{poly}}(\log n)$ if so is $|E_1|$.




